Measurements of CP-Violating Asymmetries in B0 to a1(1260)^{+-} pi^{-+} Decays

We present measurements of CP-violating asymmetries in the decay B0 -> a_1(1260)^{+-} pi^{-+} with a_1(1260)^{+-} -> pi^{-+} pi^{+-} pi^{+-}. The data sample corresponds to 384 million B B-bar pairs collected with the BaBar detector at the PEP-II asymmetric B-factory at SLAC. We measure the CP-violating asymmetry A^{a_1 \pi}_{CP}=-0.07+-0.07+-0.02, the mixing-induced CP violation parameter S_{a_1 \pi}= 0.37 +-0.21+-0.07, the direct CP violation parameter C_{a_1 \pi}=-0.10+-0.15+-0.09, and the parameters \Delta C_{a_1 \pi}=0.26+-0.15+-0.07 and \Delta S_{a_1\pi}=-0.14+-0.21+-0.06. From these measured quantities we determine the angle \alpha_{\rm eff}= 78.6^{\circ} +- 7.3^{\circ}.

==> abstract.tex <==
We present measurements  of CP-violating asymmetries in the decay 
B0 -> a_1(1260)^{+-} pi^{-+} with a_1(1260)^{+-} -> pi^{-+} pi^{+-} pi^{+-}.
The data sample corresponds to  384 million  B B-bar  pairs  
collected with the BaBar detector at the PEP-II asymmetric B-factory
at SLAC. We measure the CP-violating asymmetry
A^{a_1 \pi}_{CP}=-0.07+-0.07+-0.02, the mixing-induced CP
violation parameter S_{a_1 \pi}= 0.37 +-0.21+-0.07, the direct CP
violation parameter C_{a_1 \pi}=-0.10+-0.15+-0.09, and the parameters
\Delta C_{a_1 \pi}=0.26+-0.15+-0.07 and \Delta S_{a_1\pi}=-0.14+-0.21+-0.06.
From these measured quantities we determine the angle \alpha_{\rm
eff}= 78.6^{\circ} +- 7.3^{\circ}.


